Single-Forward-Step Projective Splitting: Exploiting Cocoercivity

This work describes a new variant of projective splitting for solving maximal monotone inclusions and complicated convex optimization problems. In the new version, cocoercive operators can be processed with a single forward step per iteration. In the convex optimization context, cocoercivity is equivalent to Lipschitz differentiability. Prior forward-step versions of projective splitting did not fully exploit cocoercivity and required two forward steps per iteration for such operators. Our new single-forward-step method establishes a symmetry between projective splitting algorithms, the classical forward-backward splitting method (FB), and Tseng's forward-backward-forward method (FBF). The new procedure allows for larger stepsizes for cocoercive operators: the stepsize bound is $2\beta$ for a $\beta$-cocoercive operator, the same bound as has been established for FB. We show that FB corresponds to an unattainable boundary case of the parameters in the new procedure. Unlike FB, the new method allows for a backtracking procedure when the cocoercivity constant is unknown. Proving convergence of the algorithm requires some departures from the prior proof framework for projective splitting. We close with some computational tests establishing competitive performance for the method.

==> Lipschitz.tex <==
\section{A Procedure for Lipschitz-Continuous Operators}
\label{secLip}
\subsection{The Procedure}

Suppose that for some subset $\IL\subseteq\{1,\ldots,n\}$, the operator $B_i$ is merely Lipschitz-continuous (but not cocoercive). This setting was considered in our previous work, \cite{johnstone2018projective}, where a two-forward-step procedure was developed. We will show in this section that this older procedure and the one developed in this paper that uses one forward step can be used together in one ``master algorithm". For cocoercive operators, we can use the new procedure which requires only one forward step. For merely Lipschitz-continuous operators, we can use the old procedure from \cite{johnstone2018projective}. It turns out that the two procedures work together and the proof combines them seamlessly. 

For simplicity, we will not develop backtracking, even though it can be used in both procedures. Note also that the resolvents for $i\in\IL$ can be evaluated approximately using a relative error criterion developed in \cite{johnstone2018projective}, but we will not utilize this here. 
One departure from \cite{johnstone2018projective} is that the update on Line \ref{lineLip} in Algorithm \ref{AlgWithLip} combines the forward steps and resolvent together into one update. This feature was first used in \cite{tran2015new}. In this form there is a connection between the two-forward-step procedure and Tseng's modified forward-backward splitting method \cite{tseng2000modified} for the special case of $n=1$ with $\IL = \{1\}$. Tseng's method is almost a special case of projective splitting, albeit with a different stepsize. We show this in Section \ref{secTseng} below. 

Comparing lines \ref{lineLip} and \ref{lineCoco} in Algorithm \ref{AlgWithLip}, we see clearly the advantage of the new procedure. If we have cocoercivity, the new procedure on line \ref{lineCoco} can reuse an old forward evaluation and only needs one new forward evaluation --- $B_i x_i^k$. On the other hand, the old procedure must compute two forward steps --- $B_i G_i z^k$ and $B_i x_i^k$ --- at each iteration. Thus the new procedure effectively halves the computation per iteration in this part of the algorithm, since the forward evaluation is typically the most costly part (assuming a simple resolvent w.r.t.~$A_i$). Furthermore, the new procedure allows larger stepsizes than the old procedure. %However, if $B_i$ is merely Lipschitz continuous but not cocoercive, we can still use the old procedure. 

\begin{algorithm}[h!]
	\DontPrintSemicolon
	\SetKwInOut{Input}{Input}
	\SetKwFunction{projectToHplane}{projectToHplane}
	\Input{$(z^1,{\bf w}^1)\in \boldsymbol{\mathcal{H}}$, $(x_i^0,b_i^0)\in\calH_i^2$.}
	\For{$k=1,2,\ldots$}
	{   
		
		\For{$i=1,2,\ldots, n$}
		{			
			\eIf{$i\in\IL$}
			{							
				$x_i^k +\rho_i^k a_i^k = G_i z^k - \rho_i^k(B_i G_i z^k - w_i^k):\, a_i^k\in A_i x_i^k$\label{lineLip}\;

			}
		   {
				$x_i^k + \rho_i^k a_i^k = \alpha_i^k G_i z^k+(1-\alpha_i^k)x_i^{k-1} -\rho_i^k(b_i^{k-1} - w_i^k):\, a_i^k\in A_i x_i^k$\label{lineCoco}\;		              	   
		   }
   			$b_i^k = B_i x_i^k$\label{lineBup}\; 
	   		$y_i^k = a_i^k+b_i^k$\label{lineYup}\;  
		}    
		$(\pi_k, z^{k+1}, {\bf w}^{k+1})$ $\leftarrow$ \projectToHplane{$z^k, {\bf w}^k, \{x_i^k,y_i^k\}_{i=1}^n$,$\beta_k$}\;
		
		\If{$\pi_k=0$}
		{
			\Return $z^{k+1}$\;
			
		} 
	}
	\caption{Projective Splitting with Lipschitz Continuous and Cocoercive Operators}
	\label{AlgWithLip}
\end{algorithm}

\subsection{Analysis}

The strategy for proving convergence of the iterates of Algorithm \ref{AlgWithLip} is as follows. As before, we utilize Lemma \ref{lemStrat}. In order to get there, we first estabish that $(x_i^k,y_i^k)$ are bounded for $i\in\IL$. We then estabish a far simpler ``Ascent Lemma" for $\varphi_{i,k}(p^k)$ with $i\in\IL$ than is possible for $i\in\IL^c$. Finally, we show how this can be used within the argument of Lemma \ref{lemFirstBiggy} to show $y_i^k - w_i^k\to 0$ and $G_i z^k - x_i^k\to 0$ for $i\in\IL$, which is all we need alongside prior results to use Lemma \ref{lemStrat}.

\begin{assumption}\label{assLip}
For Problem \eqref{prob1} Assumption \ref{assMono} holds with the following change: For $i\in\IL\subseteq\{1,\ldots,n\}$ the operators $B_i$ are merely $L_i$-Lipschitz continuous and not necessarily cocoercive. 
\end{assumption}

\begin{assumption}
\label{assLipStep}
For $i\in\IL^c$ Assumption \ref{assStep} holds. For $i\in\IL$, there exists $0<\urho_i\leq\orho_i$ s.t. 
\begin{align*}
(\forall k\geq 1):\quad 
\urho_i
\leq 
\rho_i^k
\leq 
\orho_i
<
\frac{1}{L_i}.
\end{align*}
\end{assumption}

In lemmas \ref{lemLipBounded}--\ref{lemLipAscent} below, assumptions \ref{assBasic}, \ref{assAv}, \ref{assLip}, and \ref{assLipStep} are in effect and won't be explicitly stated. 

\begin{lemma}\label{lemLipBounded}
For $i\in\IL$, $(x_i^k,y_i^k)$ are bounded.	
\end{lemma}
\begin{proof}
The right hand side in line \ref{lineLip} is bounded by Lemma \ref{lemProj} along with the facts that $\rho_i^k$ and $\|G_i\|$ are bounded. Therefore $x_i^k +\rho_i^k a_i^k$ is bounded. Now we can follow the argument of Lemma 10 in \cite{eckstein2017simplified} to argue that $x_i^k$ and $a_i^k$ are bounded. Therefore $b_i^k$ is bounded by the continuity of $B_i$ and $y_i^k$ is bounded by line \ref{lineYup}. 
\end{proof}

\begin{lemma}\label{lemLipAscent}
For $i\in\IL$, and $k\geq 1$:
$\varphi_{i,k}(p^k)\geq \left((\rho_i^k)^{-1}-L_i\right)\|G_i z^k - x_i^k\|^2$.
\end{lemma}
\begin{proof}
A more general result than this was proved in Lemma 12 of \cite{johnstone2018projective} and Proposition 14 of \cite{eckstein2017simplified}. For completeness, we include the argument here. We write
\begin{align*}
\varphi_{i,k}(p^k)
&=
\langle 
G_i z^k - x_i^k,y_i^k-w_i^k
\rangle 
\\
&=
\langle 
G_i z^k - x_i^k,a_i^k+b_i^k-w_i^k
\rangle 
\\
&=
\langle 
G_i z^k - x_i^k,a_i^k+B_i G_i z^k-w_i^k
\rangle 
+
\langle 
G_i z^k - x_i^k,B_i x_i^k-B_i G_i z^k
\rangle 
\\
&\geq 
\langle 
G_i z^k - x_i^k,a_i^k+B_i G_i z^k-w_i^k
\rangle 
-
L_i\|G_i z^k - x_i^k\|^2
\\
&=
\left((\rho_i^k)^{-1}-L_i\right)\|G_i z^k - x_i^k\|^2
\end{align*}
where in the inequality we used Cauchy-Schwarz followed by Lipschitz continuity of $B_i$ to simplify the second term, and in the final equation we rearranged line \ref{lineLip} to
$$
a_i^k+B_i G_i z^k-w_i^k = (\rho_i^k)^{-1}(G_i z^k - x_i^k)
$$
and substituted this into the first term. 
\end{proof}

\begin{lemma}
\label{thmLip}
Suppose assumptions \ref{assBasic}, \ref{assAv}, \ref{assLip}, and \ref{assLipStep} hold. Then the conclusions of Theorem \ref{thmMain} follow for Algorithm \ref{AlgWithLip}.
\end{lemma}
\begin{proof}
	Finite convergence is dealt with as before. From now on assume the algorithm produces infinitely many iterations. 
For $i\in \IL$, it is far simpler to establish that $\liminf \varphi_{i,k}(p^k)\geq 0$. In fact Lemma \ref{lemLipAscent} estabishes the far stronger result: 
\begin{align}\label{eqTooEasy}
\varphi_{i,k}(p^k)\geq \left((\rho_i^k)^{-1}-L_i\right)\|G_i z^k - x_i^k\|^2\geq 0 
\end{align}
for all $k\geq 1$. 
We will use this to modify the arguments in Lemma \ref{lemFirstBiggy}. For $i\in\IL$ define 
$$
r_i^k = 
\varphi_{i,k}(p^k)- \left((\rho_i^k)^{-1}-L_i\right)\|G_i z^k - x_i^k\|^2\geq 0.
$$
Whereas for $i\in\IL^c$, define $r_i^k$ as before in \eqref{rdef}. 
Then \eqref{eqSumr} becomes
\begin{align}
\sum_{i=1}^n r_i^k
=
\varphi_{k}(p^k)
-
\sum_{i\in\IL^c}
\frac{\rho_i^{k+1}}{2\alpha_i^{k+1}}
\|y_i^k - w_i^k\|^2
-
\sum_{i\in\IL}
\left((\rho_i^k)^{-1}-L_i\right)\|G_i z^k - x_i^k\|^2.
\nonumber
\end{align}
We may again establish $\liminf r^k_i\geq 0$. For $i\in\IL^c$, the argument is unchanged. For $i\in\IL$, we can just use \eqref{eqTooEasy}. Therefore we may repeat the arguments in Lemma \ref{lemFirstBiggy} going from \eqref{eqsumrLow} to \eqref{eqEndGreat} which leads to the conclusion: $\varphi_k(p^k)\to 0$. Thus, as before we get $y_i^k-w_i^k\to 0$ for $i\in\IL^c$. For $i\in\IL$, we get $G_i z^k - x_i^k\to 0$. 
Furthermore for $i\in\IL$
\begin{align*}
\|y_i^k - w_i^k\|
&=
\|a_i^k+b_i^k - w_i^k\|
\\
&\leq 
\|a_i^k+B_i G_i z^k - w_i^k\|+\|b_i^k - B_i G_i z^k\|
\\
&=
(\rho_i^k)^{-1}\|G_i z^k - x_i^k\|+\|B_i x_i^k - B_i G_i z^k\|
\\
&\leq 
((\rho_i^k)^{-1}+L_i)\|x_i^k-G_i z^k\|\to 0. 
\end{align*}
For $i\in\IL^c$, lemmas \ref{lemFirstX} and
\ref{lemSecondX} are proved as before. 
Thus the conditions required in Lemma \ref{lemStrat} are met. 
\end{proof}
\subsection{A Connection to Tseng's Modified Forward-Backward Splitting Method}
\label{secTseng}
Suppose $n=1$ and $\IL = \{1\}$, so that we are solving
\begin{align*}
0\in Az + B z 
\end{align*}
where $B\triangleq B_1$ is monotone and Lipschitz continuous (but not necessarily cocoercive) and $A\triangleq A_1$ is maximal monotone.  
In this case $w_1^k = 0$ since $n=1$. Furthermore note that $G_1=I$.
Then the updates on lines \ref{lineLip} and \ref{lineYup} of Algorithm \ref{AlgWithLip} become 
\begin{align}
\label{eqTseng1}
x^k &= J_{\rho^k A}(z^k - \rho^k B z^k)
\\\nonumber 
y^k &= B x^k - B z^k + (\rho^k)^{-1}(z^k  - x^k)
\end{align}
where we have dropped the unnecessary subscript and written $x^k\triangleq x_1^k$, $y^k\triangleq y_1^k$, and $\rho^k\triangleq \rho_1^k$. 
Now 
\begin{align*}
\frac{\varphi_k(p^k)}{\|\nabla\varphi_k\|^2_\gamma}
=
\frac{\gamma\langle z^k - x^k,y^k\rangle}{\|y^k\|^2}
=
\frac{\gamma\langle \rho^k y^k+\rho^k(B z^k - B x^k),y^k\rangle}{\|y^k\|^2}
=
\gamma\rho^k
\left(
1
+
\frac{\langle B z^k - B x^k,y^k\rangle}{\|y^k\|^2}
\right).
\end{align*}
Then the projection update on line \ref{lineZproj} of Algorithm \ref{AlgProjUpdate} becomes 
\begin{align}
z^{k+1}
&=
z^k
-
\frac{\varphi_k(p^k)}{\gamma\|\nabla\varphi_k\|^2_\gamma} y^k
\nonumber\\
&=
z^k
-
\tilde{\rho}^k
\left(
B x^k - B z^k + (\rho^k)^{-1}(z^k  - x^k)
\right)
\nonumber\\\label{eqTseng2}
&=
\left(1-\frac{\tilde{\rho}^k}{\rho^k}\right)z^k +\frac{\tilde{\rho}^k}{\rho^k} x^k - \tilde{\rho}^k(B x^k - B z^k)
\end{align}
where
\begin{align*}
\tilde{\rho}^k\triangleq 
\rho^k
\left(
1
+
\frac{\langle B z^k - B x^k,y^k\rangle}{\|y^k\|^2}
\right).
\end{align*}
Combining \eqref{eqTseng1} and \eqref{eqTseng2} yields the method:
\begin{align*}
x^k &= J_{\rho^k A}(z^k - \rho^k B z^k)
\\
z^{k+1}
&=
\left(1-\frac{\tilde{\rho}^k}{\rho^k}\right)z^k +\frac{\tilde{\rho}^k}{\rho^k} x^k - \tilde{\rho}^k(B x^k - B z^k).
\end{align*}
If $\tilde{\rho}^k=\rho^k$ then this reduces to Tseng's method \cite{tseng2000modified} without the second projection onto the set $X$. However, $\tilde{\rho}^k$ will not equal $\rho^k$ in general, so  projective splitting in this case only resembles Tseng's method but is not the same. 

It is worth noting that projective splitting in this case only requires one resolvent evaluation w.r.t.~$A$ at each iteration, like Tseng's method. This is in contrast with the extragradient method \cite{korpelevich1977extragradient}, which requires two. 


==> NotationMathPrelims.tex <==



%% JE == again, too standard to spend space on
% An $L$-Lipschitz continuous operator $B$ for some $L\geq 0$ satisfies
% $$
% \forall x,y\in \text{dom}(B): \|Bx-By\|\leq L\|x-y\|
% $$
% and is clearly single-valued. 


==> backTrack.tex <==
%!TEX root = coconuts.tex
\subsection{Backtracking Linesearch}\label{secBackTrack}













==> extensions.tex <==
\section{To do}
\begin{itemize}
\item XX
\end{itemize}


==> portfolio-old.tex <==
\newcommand{\onef}{\texttt{ps1fbt}}
\newcommand{\twof}{\texttt{ps2fbt}}
\newcommand{\ada}{\texttt{ada3op}}
\newcommand{\cp}{\texttt{cp-bt}}
\newcommand{\tseng}{\texttt{tseng-pd}}
\newcommand{\frb}{\texttt{frb-pd}}



\section{Numerical Experiments}
\subsection{Methods Tested}
All numerical experiments are implemented in python (\texttt{numpy}) on a Linux Ubuntu system XX. We restricted our attention to algorithms with comparable features, complexity, and benefits to our proposed method. As such we only considered methods that
\begin{itemize}
\item are first-order and ``fully split" the problem,
\item  do not (either approximately or exactly) invert a linear system at each iteration or before the first iteration,
\item do not approximate difficult resolvent calculations,
\item do not ``smooth " nonsmooth functions in some way, and
\item incorporate a backtracking linesearch and so avoid computing the Lipschitz constant of the gradient. 
\end{itemize}
Of course there are many effective algorithms which could have been considered but do not satisfy one of these requirements. However since these properties are important ingredients in making algorithms scalable and simple to use, we chose to focus on this subset.

We compare the one-forward-step projective splitting algorithm with backtracking of this paper given in Algorithm \ref{AlgfullWithBT} (which we call \texttt{ps1fbt}) with the following methods: 
\begin{enumerate}
	\item The two-forward-step projective splitting algorithm with backtracking we developed in \cite{johnstone2018projective} (\texttt{ps2fbt}). 
	\item The adaptive three operator splitting algorithm of \cite{pedregosa2018adaptive} (\texttt{ada3op}) (they use adaptive to mean ``backtracking linesearch"). 
	\item 
	The backtracking linesearch variant of the Chambolle-Pock primal-dual splitting method \cite{malitsky2018first} (\cp).
	\item The algorithm of \cite{combettes2012primal}. Since this is an instance of Tseng's method applied to an appropriate primal-dual ``monotone + skew" inclusion, we call it \tseng. In order to achieve good performance with \tseng\space we had to incorporate a diagonal preconditioner ()as was proposed in \cite{vu2013variable}). 
	\item The recently-proposed forward-reflected-backward method \cite{tam2018forward} which, like \tseng, may be applied to the same ``monotone+skew" primal-dual inclusion. Since this is also a primal-dual method we call it \frb. As with \tseng, we had to use a preconditioner to get good performance with \frb. 
\end{enumerate}
%Note that all these methods satisfy the above requirements. 
% The main hypothesis to test is whether \onef \space outperforms \twof, but we are also concerned with how \onef\space compares with \ada, \cp, and \tseng, as these are more established first-order splitting methods. 

\subsection{Portfolio Selection}\label{secPort}
Consider the following optimization problem:
\begin{align}\label{propPort} 
\min_{x\in\rR^d}
F(x)\triangleq 
x^\top Q x
\quad \text{s.t.}\quad 
m^\top x \geq r,\quad 
\sum_{i=1}^d x_i = 1,x_i\geq 0
\end{align}
where $Q\succeq 0$, $r>0$, and $m\in\rR^d_+$. 
This optimization model arises in Markowitz portfolio theory. We chose this particular problem because it features two constraint sets (a hyperplane and the simplex) for which it is easy to project onto each individually but hard to project onto their intersection. This makes it difficult to apply first-order methods such as ISTA/FISTA \cite{beck2009fast} as they can only handle one constraint (they cannot fully split the problem). On the other hand projective splitting can handle an arbitrary number of constraints. The most applicable operator splitting method beyond projective splitting for this problem is three operator splitting \cite{davis2015three} and its backtracking variant \cite{pedregosa2018adaptive}. We consider a fairly large instance of this problem so that standard interior point methods (for example those in the CVXPY package) are not very competitive and the first-order methods are the best choice. Furthermore, backtracking varieties are preferable for large problems as they avoid the need to estimate the largest eigenvalue of $Q$. 

A random instance of \eqref{propPort} is created as follows. We set $d=10,000$ so this is a relatively large instance of the problem. We generate a matrix $Q_0$ of size $d\times d$ with each entry drawn from $\calN(0,1)$. The matrix $Q$ is then formed as $Q_0 Q_0^\top$ which is guaranteed to be positive-semidefinite. A vector $m$ of length $d$ is generated with entries uniformly distributed between $0$ and $100$. The constant $r$ is set to $(1/2)\sum_{i=1}^d m_i/d$.
All methods are initialized at the same point: $[1~1~\ldots~1]^\top/d$, with the same initial trial stepsize of $1$. 

To convert \eqref{propPort} to a monotone inclusion we set $A_1 = N_{C_1}$ where $N_{C_1}$ is the normal cone of the simplex: $C_1 = \{x\in\rR^d:\sum_{i=1}^d x_i=0,x_i\geq 0\}$. We set $B_1 = 2Qx$ which is the gradient of the objective function and is cocoercive (and Lipschitz-continuous). Finally $A_2 = N_{C_2}$ where $C_2 = \{x:m^\top x\geq r\}$. 
Note that the resolvents w.r.t.~$N_{C_1}$ and $N_{C_2}$ (that is, the projections onto $C_1$ and $C_2$) are easily computed in $O(d)$ operations. 
With this notation we write the  monotone inclusion as finding $z\in\rR^d$ s.t.
\begin{align}\label{probPortMono}
0\in A_1 z + B_1 z + A_2 z
\end{align} 
which is an instance of \eqref{prob1} with $n=2$ and $G_1=G_2=I$. 
The constraint qualification s.t.~\eqref{propPort} and \eqref{probPortMono} are equivalent is merely that $\text{ri } C_1\cap\text{ri } C_2$ is nonempty \cite[Cor.~27.6(b)]{bauschke2011convex} which is guaranteed by how we choose $r$.% We can now apply our three methods to solving \eqref{probPortMono}. 

For \texttt{ps1fbt} and \texttt{ps2fbt} we set $\gamma=10$ and $\rho_2^k$ fixed to $0.1$. The performance of these algorithms was sensitive to the choice of these parameters and they needed to be tuned. For both methods $\rho_1^k$ is computed by backtracking with first initial guess $\hat{\rho}_1^1=1$ and after this the initial guess is set to $\hat{\rho}_1^k = \rho_1^{k-1}$. For the averaging parameters in \texttt{ps1fbt} we used $\alpha_1^k$ fixed to $0.1$ and $\alpha_2^k$ fixed to $1$ (which is allowed because $L_2=0$). The backtracking stepsize decrement factor $\delta=0.9$ for all three algorithms. For \texttt{ps1fbt} we set $\hat{\theta}_1 = x_1^0$ and $\hat{w}_1 =2 Q x_1^0$. 


\begin{figure}
\includegraphics[width=0.5\textwidth]{func_vs_iter}	
\includegraphics[width=0.5\textwidth]{func_vs_time}	
\caption{Results for solving \eqref{propPort}: portfolio optimization. We compare three methods: 1.~\texttt{ps1fbt} the method proposed here in Algorithm \ref{AlgfullWithBT}, 2.~\texttt{ps2fbt} our two-forward-step method of \cite{johnstone2018projective}, and 3.~\texttt{ada3op} the adaptive three operator splitting method \cite{pedregosa2018adaptive}. The left plots the relative optimality gap: $(F(x)-F^*)/F^*$ where $F^*$ is the optimal value of the problem vs number of iterations. The right plots this against elapsed time.}
\label{figPlot}
\end{figure}

The results of the experiment are plotted in Figure \ref{figPlot}. We ran each algorithm for $1000$ iterations. The optimal value $F^*$ was estimated by the smallest final function value achieved by any algorithm. 
We compare the function values of $x_1^k$ computed by \texttt{ps1fbt} and \texttt{ps2fbt} and $x_t$ computed on Line 3 of \cite[Algorithm 1]{pedregosa2018adaptive} for \texttt{ada3op}. For this particular experiment, all three of these variables were feasible for all iterations, so we only compare the algorithms in terms of function value convergence. 
On the left we see a comparison of the three methods in terms of the number of iterations. The convergence rates of \texttt{ps1fbt} and \texttt{ada3op} are comparable and \texttt{ps2fbt} is slightly slower. However \texttt{ps1fbt} is doing less work than the other methods at each iteration. 
Since $d$ is large and $Q$ is a large dense matrix, multiplication by $Q$ is the dominant computation at each iteration for each algorithm.
While \texttt{ps1fbt} does a minimum of one forward evaluation of $B_1x = 2Q x$ at each iteration, \texttt{ps2fbt} must do two. \texttt{ada3op} must also do at least two: one to compute $\nabla F(z_t)$ on line 3 and one to compute $F(x_{t+1})$ on line 4 of \cite[Algorithm 1]{pedregosa2018adaptive}. This difference is evident in the right plot in Figure \ref{figPlot} where we see that the total running time of \texttt{ps1fbt} is smaller than the other two algorithms. 

This experiment demonstrates that, by exploiting the cocoercivity of the operator $B_1$, our new one-forward-step procedure outperforms the old two-forward-step procedure which only utilizes Lipschitz continuity. It also appears to outperform \texttt{ada3op} in terms of the number of $Q$-multiplies and subsequent running time. We believe this is mostly because \texttt{ada3op} is obliged to check the value $F(x_t)$ at each iteration and therefore must do two multiplies. However we should note that \texttt{ada3op} has the advantage that it has fewer tuning parameters than our method. 



==> prepResults.tex <==
\subsection{Preparatory Results}







\begin{assumption}
	\label{assBasic}
	There exists $0<\ubeta\leq\obeta<2$ s.t. for all $k\geq 1$: $\ubeta\leq \beta_k\leq \obeta$. The constant $\gamma$ is positive. 
\end{assumption}

\begin{lemma}\label{lemIsProject}
	Suppose that assumptions \ref{assMono} and \ref{assBasic} hold.
	Then
	\begin{enumerate}
		\item The sequence $\{p^k\}=\{(z^k,w_1^k,\ldots,w_{n-1}^k)\}$ is bounded.
		\item If the algorithm never terminates via line \ref{lineReturn}, $p^k - p^{k+1}\to 0$.
		\item Furthermore $z^k - z^{k-1}\to 0$ and $w_i^k - w_i^{k-1}\to 0$ for $i=1,\ldots n$.  
		\item If the algorithm never terminates via line \ref{lineReturn} and there exists $M\geq 0$ s.t.~$\|\nabla\varphi_k\|\leq M$ for all $k\geq 1$, then $\limsup_{k\to\infty}\varphi_k(p^k)\leq 0$. 
	\end{enumerate}
\end{lemma}
\begin{proof}
Parts 1--3 are proved in lemmas 2 and 6 of \cite{johnstone2018projective}. Part 4 can be found in Part 1 of the proof of Theorem 1 in \cite{johnstone2018projective}.
\end{proof}

==> projSplitBasics.tex <==
\subsection{The Basics of Projective Splitting}

==> projectMethods.tex <==
\section{Mathematical Preliminaries}
\label{sec_math_prelim}
\subsection{A Generic Linear Separator-Projection Method}

Let the real Hilbert space $\boldsymbol{\mathcal{H}}$ have inner
product $\langle\cdot,\cdot\rangle_{\bcalH}$ and norm $\|\cdot\|_{\bcalH}$. A
generic  linear separator-projection method for finding a point in the closed
and convex set $\calS\subseteq\boldsymbol{\mathcal{H}}$ is given in Algorithm
\ref{AlgGenericProject}.

\begin{algorithm}[h!]\label{AlgGenericProject}
	\DontPrintSemicolon
	\SetKwInOut{Input}{Input}
\Input{$p^1$, $0<\underline{\beta}\leq\overline{\beta}<2$}
	\caption{Generic linear separator-projection method for finding a point in a closed and convex set $\calS\subseteq\boldsymbol{\mathcal{H}}$.}
	\label{AlgAbstractProject}
	\For{$k=1,2,\ldots,$}{
	Find an affine function $\varphi_k$ such that $\nabla\varphi_k\neq 0$ and
	    $\varphi_k(p)\leq 0$ for all $p\in \calS$. \;
	Choose $\beta_k\in[\underline{\beta},\overline{\beta}]$\label{eqProjectUpdatem1}\;
	$p^{k+1} = p^k - 
	\frac{\beta_k\max\{0,\varphi_k(p^k)\}}
	{\|\nabla\varphi_k\|_{\bcalH}^2}
	\nabla\varphi_k$
	\label{eqProjectUpdate}\;
 }
\end{algorithm}
%$\hat{p}_k = \text{projection of }p^k\text{ onto }\{p:\varphi_k(p)\leq 0\}$
%using the norm: $\|\cdot\|_{\bcalH}$\; $p^{k+1}=  (1-\beta_k)p^k + \beta_k
%\hat{p}_k$

The update on line~\ref{eqProjectUpdate} is the $\beta_k$-relaxed projection of $p^k$
onto the halfspace $\{p:\varphi_k(p) \leq 0\}$ using the norm
$\|\cdot\|_{\bcalH}$. In other words, if $\hat{p}^k$ is the projection onto
this halfspace, then the update is $p^{k+1} = (1-\beta_k)p^k +
\beta_k\hat{p}^k$. Note that we define the gradient $\nabla\varphi_k$ with
respect to the inner product $\langle\cdot,\cdot\rangle_{\bcalH}$, meaning we
can write
$$
(\forall p,\tilde{p}\in\bcalH):\quad\varphi_k(p) = \langle\nabla\varphi_k,p - \tilde{p}\rangle_{\bcalH} + \varphi_k(\tilde{p}).
$$

We will use the following well-known properties
of algorithms fitting the template of Algorithm~\ref{AlgGenericProject}; see for example~\cite{combettes2000fejerXX,eckstein2008family}:
\begin{lemma} \label{lemProj}
Suppose $\calS$ is closed and convex. Then for Algorithm \ref{AlgAbstractProject},
	\begin{enumerate}
		\item The sequence $\{p^k\}$ is bounded.
		\item $\|p^k - p^{k+1}\|_{\bcalH}\to 0$;
	%	\item If all weak limit points of $\{p^k\}$ are in $\calS$, then
	%	$p^k$ converges weakly to some point in $\calS$.
		\item If there exists $M\geq 0$ s.t.~$\|\nabla\varphi_k\|_{\bcalH}\leq M$ for all $k\geq 1$, then $\limsup_{k\to\infty}\varphi_k(p^k)\leq 0$. 
	\end{enumerate}\label{propFejer}
\end{lemma}
\begin{proof}
The first two results are standard for projection methods and can be found in \cite{combettes2000fejerXX,eckstein2008family}. For the final point
\begin{align*}
0 
&= 
\lim_{k\to\infty}
\|p^{k+1}-p^k\|_{\bcalH}
\\
&=
\lim_{k\to\infty}
	\frac{\beta_k\max\{0,\varphi_k(p^k)\}}
{\|\nabla\varphi_k\|_{\bcalH}}
\\
&\geq 
\lim_{k\to\infty}
	\frac{\underline{\beta}\max\{0,\varphi_k(p^k)\}}
{M}
\end{align*}
from which the result follows. 
\end{proof} 





==> rare.tex <==

\newcommand{\calT}{\mathcal{T}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\subsection{Rare Feature Selection}\label{sec_rare}
In \cite{2018arXiv180306675Y}, the problem of utilizing rare features in
machine learning problems was studied. In many applications, certain features are
rarely nonzero, making it hard to estimate their
coefficients accurately. Despite this, these features can be highly
informative, and the standard practice of discarding them is wasteful. The
technique in \cite{2018arXiv180306675Y} overcomes this difficulty by making
use of  an auxiliary tree data structure $\calT$ describing the relatedness of
features. Each leaf of the tree is a feature and two features' closeness on
the tree measures how ``related" they are. Closely related features can then
be aggregated (summed) so that more samples are captured, increasing the
accuracy of the estimate for a single coefficient for the aggregated features.


To solve this aggregation and fitting problem automatically,
\cite{2018arXiv180306675Y} introduced the following generalized regression
problem:
\begin{align}\label{eqTheirTrip}
\min_{\substack{\beta_0\in \rR \\ \bbeta\in \rR^d \\ \bgamma\in \rR^{|\calT|}}}
\left\{ \left.
\frac{1}{2n}\|\beta_0 e + X\bbeta - y\|_2^2
+
\lambda 
\big(
\mu\|\bgamma_{-r}\|_1
+
(1-\mu)\|\bbeta\|_1
\big)
~ \right| \bbeta = H\bgamma 
\right\}
\end{align}
where $X\in \rR^{n\times d}$ is the data matrix, $y\in\rR^n$ is the target
(response) vector, $\bbeta\in\rR^d$ are the feature coefficients, $e\in\rR^n$
has all elements equal to $1$, and $\beta_0\in\rR$ is an offset. Each
$\bgamma_i$ is associated with a node of the similarity tree $\calT$ and
$\bgamma_{-r}$ means all nodes except the root. The matrix
$H\in\rR^{d\times|\calT|}$ contains a $1$ in positions $i,j$ for which feature
$i$ corresponds to a leaf of $\calT$ that is descended from node $j$, and
elsewhere contains zeroes. $H$ thus fuses coefficients together in the
following way: if $\bgamma_i$ is nonzero for a node $i$ and all descendants of
$\bgamma_i$ in $\calT$ are $0$, then all coefficients on the leaves which are
descendant from $\bgamma_i$ are equal (see \cite[Sec.
3.2]{2018arXiv180306675Y} for more details). The $\ell_1$ norm on $\bgamma$
enforces sparsity of $\bgamma$, which in turn fuses together coefficients in
$\bbeta$ associated with similar features. The $\ell_1$ norm on $\bbeta$
itself additionally enforces sparsity on these coefficients, which is also
desirable.

In \cite{2018arXiv180306675Y}, \eqref{eqTheirTrip} is solved by a specialized
application of the ADMM. The implementation involves precomputing the SVDs of
$X$ and $H$, and so does not fall within the scope of the methods considered in
our experiments (it does not fully split the problem). Instead, we solve \eqref{eqTheirTrip} by simply eliminating
$\bbeta$, so that it becomes
\begin{align}\label{eqOurTrip}
F^*\triangleq \min_{\substack{\beta_0\in \rR \\ \bgamma\in \rR^{|\calT|}}} \!\!
%F(\bgamma,\beta_0)\triangleq 
\left\{
\frac{1}{2n}
\|
\beta_0 e +
X H \bgamma  - y
\|_2^2
+
\lambda 
\left(
\mu\|\bgamma_{-r}\|_1
+
(1-\mu)\|H\bgamma\|_1
\right)
\right\}.
\end{align}
This problem may be formulated as a special case of \eqref{ProbOpt} with 
\begin{align*}
f_1(t) &= \lambda (1-\mu)\|t\|_1 & h_1(t) &= 0 & G_1 &= H \\
f_2(\bgamma,\beta_0) &=\lambda \mu\|\bgamma_{-r}\|_1 & 
h_2(\bgamma,\beta_0) &=\frac{1}{2n} \|
\beta_0 e +
X H \bgamma  - y
\|_2^2
& G_2 &= I.
\end{align*}
Note that $h_2$ is Lipschitz differentiable and $f_1$ (and $f_2$) have
easily-computed proximal operators. Because of the presence of the matrix $G_1 = H$,
\ada\space cannot easily be applied to this problem, since the proximal
operator of the function $\bgamma \mapsto \|H\bgamma\|_1$ cannot be computed
in a simple way.  All other methods, namely \onef, \twof, \cp, \tseng, and
\frb, may still be applied.

We apply this model to the TripAdvisor hotel-review dataset developed 
in~\cite{wang2010latent} and~\cite{2018arXiv180306675Y}\footnote{TripAdvisor data is available at \url{https://github.com/yanxht/TripAdvisorData} or through our repository at \url{https://github.com/projective-splitting/coco}}.
The response variable was the overall hotel review,
in the set $\{1,2,3,4,5\}$. The features were the counts of certain
adjectives in the review. Many adjectives were very rare, with $95\%$ of the
adjectives appearing in less than $5\%$ of the reviews. The authors
of~\cite{2018arXiv180306675Y} constructed a similarity tree using information
from word embeddings and emotion lexicon labels. In the end, there were
$7,\!573$ adjectives from the $209,\!987$ reviews and the tree $\calT$ had
$15,\!145$ nodes. They withheld $40,\!000$ examples for a test set. The
$169,\!987\times 7,\! 573$ design matrix $X$ was sparse, having only $0.32\%$
nonzero entries. The $7,\! 573\times 15,\!145 $ matrix  $H$ arising from the
similarity tree $\calT$ was also sparse, having $0.15\%$ nonzero entries. In
our implementation, we used the sparse matrix package \texttt{sparse} in
\texttt{scipy}.

In practice, one typically would solve \eqref{eqOurTrip} for many values of $(\mu,\lambda)$ and then choose the final model based on cross validation. To assess the computational performance of the tested methods, we solve three representative examples corresponding to sparse, medium, and dense solutions. For simplicity, we fixed $\mu=0.5$. The chosen values for $\lambda$ were $\{10^{-5},10^{-2},10^{-1}\}$. 

The setup for the algorithms was the same as in the previous two examples,
except for a few differences. For backtracking, we simply set the trial stepsize at each iteration equal
to the previously discovered stepsize, as increasing it at each iteration did not provide any empirical benefit. However \cp\space performed better with increasing trial stepsize so we used the same
scheme as before. For \onef\space and \twof, setting $\rho_1^k$  equal to the
discovered backtracking stepsize for the other operator from the previous
iteration: $\rho_2^{k-1}$, did not work well on this model. So instead we
fixed $\rho_1^k=1$ for \onef\space and $\rho_1^k=10$ for \twof, which
gave the best performance across the three examples. Each tested method then
has one additional tuning parameter which we hand-picked for each of the three
examples. The final values are given in table \ref{table-tune-rare}.


\begin{table}
	\centering
	\begin{tabular}{c||c|c|c|c}
		&\multicolumn{3}{c}{$\lambda$}
		\\
		&$10^{-5}$&$10^{-2}$&$10^{-1}$
		\\
		\hline	
		\hline	
		\onef\,($\gamma$)
		& $1$ & $10$ & $10^4$ 
		\\
		\hline 
		\twof\,($\gamma$) & $10^2$ & $10$ & $10^5$  
		\\
		\hline 
		\cp\, ($\beta^{-1}$) & $10$ & $10^3$ & $10^7$ 
		\\
		\hline 
		\tseng\, ($\gamma_{pd}$) & $1$ & $10^4$ & $10^6$  
		\\
		\hline 
		\frb\, ($\gamma_{pd}$) & $1$ & $10^4$ & $10^6$  
		\\
		\hline
		\hline  
	\end{tabular}
	\caption{Tuning parameters for the \eqref{eqOurTrip} applied to TripAdvisor data.}
	\label{table-tune-rare}
\end{table}

\begin{figure}
\minipage{0.32\textwidth}
\includegraphics[width=\linewidth]{dense.png}
\endminipage\hfill
\minipage{0.32\textwidth}
\includegraphics[width=\linewidth]{medium.png}
\endminipage\hfill
\minipage{0.32\textwidth}
\includegraphics[width=\linewidth]{sparse.png}
\endminipage
	\caption{Results for \eqref{eqOurTrip} applied to tripAdvisor data. From
	left to right, the values of $\lambda$ are  $\lambda=10^{-5},$
	$\lambda=10^{-2},$ and $\lambda=10^{-1}$; $\mu=0.5$ in all cases. The
	$y$-axis is relative objective error
	$\big(F(\bgamma,\beta_0)-F^*\big)/F^*$, where $F(\bgamma,\beta_0)$ is the
	objective function in~\eqref{eqOurTrip}, and the $x$-axis is elapsed
	running time in seconds.}
\label{Fig-rare}
\end{figure}

The results are shown in Figure~\ref{Fig-rare}. For the plots, the optimal
objective value $F^*$ was estimated by running \onef\space for $100,\!000$
iterations, while the plots are shown only for the first $20,\!000$ iterations
of \onef. The $x$-axis is running time excluding the time taken to actually
compute the function values for the graph. Overall, there is not a large gap
between the methods. However, \onef\space and \cp\space are slightly faster
for $\lambda=10^{-5}$,  \twof\space is slightly faster for $\lambda=10^{-2}$,
and \onef\space is slightly faster for $\lambda=10^{-1}$. Since \onef\space is
either fastest, tied fastest, or in close second position, it is arguably the
best performing algorithm overall. We suspect that the performance of
\onef\space (and \twof) could greatly improve if we were to break 
the loss function up into blocks and use the
greedy subproblem selection scheme we proposed in
\cite{johnstone2018projective}. We plan to develop this generalization for
\onef\space --- along with general asynchrony and block-iterativeness ---  in
future work.



==> restOfDefs.tex <==
%!TEX root =cocoerciveGeneralMatrices.tex
%\subsection{More Definitions}

%The Kuhn-Tucker solution set of Prob. \ref{probMono} is
%\begin{eqnarray}
%	\calS\triangleq
%	\left\{
%	(z,{\bf w})\in \calC:
%	w_i\in A_i(z),i=1,\ldots,n,w_{n+j}\in B_j(z),j=1,\ldots,m
%	\right\}\label{defS}
%\end{eqnarray}
%where ${\bf w}=(w_1,\ldots,w_{n+m})$. 
%and the ambient space is
%\begin{eqnarray*}
%	\mathcal{C} = \{(z,w_1,\ldots,w_{n+m})\in\calH^{n+m+1}:w_1+w_2+\ldots w_{n+m}=0\}.
%\end{eqnarray*}
%It can be verified that $\calS$ is convex and closed under Assumption \ref{AssMonoProb} stated below (see for example Lemma 1 of \cite{eckstein2017simplified}). 
%We will also use the space
%$$
%\calW = \left\{(w_1,w_2,\ldots,w_{n+m}):\sum_{i=1}^{m+n}w_i=0\right\}.
%$$






==> sequenceLemmas.tex <==
%!TEX root = coconuts.tex
\section{Sequence Lemma Proofs}
\subsection{Proof of Lemma \ref{lemBounddSeq}}\label{secBoundedSeq}

Recursing, we may write for any $k \geq 1$ that
\begin{align*}
a_{k+1}
&\leq 
\tau^{k}a_1 + b\sum_{i=1}^k \tau^{k-i} 
% \\
% &
\leq 
\tau^{k}a_1 + \frac{b}{1-\tau}
% \\
% &
\leq
a_1 + \frac{b}{1-\tau}.
\end{align*}	




\subsection{Proof of Lemma \ref{lemSeqConverge}}
\label{secConverge}
Since $b_k\to 0$, the sequence $\{b_k\}$ is bounded. It follows by
Lemma~\ref{lemBounddSeq} that $\{a_k\}$ is bounded. Therefore, there exists
$A\geq 0$ such that $a_k\leq A$ for all $k\geq 1$.

Fix $\epsilon>0$. Since $b_k\to 0$, we may choose $M\geq 0$ large enough so
that $b_m\leq \epsilon(1-\tau)/2$ for all $m\geq M$. We may also choose $N$
sufficiently large that $\tau^n A \leq \epsilon/2$ for all $n\geq N$. Recursing, we may now write, for all $m\geq M+1$ and $n\geq N$, that
\begin{align*}
a_{m+n}
&\leq 
\tau^n a_m
+
\sum_{i=0}^n \tau^{n-i} b_{m+i-1}
% \\
% &
\leq 
\tau^n a_m
+
\frac{1}{1-\tau}\cdot\epsilon(1-\tau)/2
% \\
% &
\leq 
\tau^n A
+
\frac{\epsilon}{2}
% \\
% &
\leq 
\epsilon.
\end{align*}
Thus, for all sufficiently large $k$, we have $a_k\leq\epsilon$. Since $a_n\geq
0$ and $\epsilon$ was selected arbitrarily, we conclude that $a_n\to 0$.

\subsection{Proof of Lemma \ref{lemBoundBelow}}
\label{secBoundedBelow}
First, since $b_k\to 0$, there exists $B\leq 0$ such that $b_k\geq B$ for all
$k\geq 1$. We now show that $r_k$ is bounded from below.  We begin by writing
\begin{align*}
r_{k+1}
&\geq \tau_k r_k + b_k
\\
&\geq 
\tau_k(\tau_{k-1} r_{k-1}+b_{k-1})+b_k
\\
&\geq 
r_1\prod_{i=1}^k\tau_i  + b_k+\tau_k b_{k-1}+\tau_k\tau_{k-1} b_{k-2}+\ldots
         + \left(\prod_{i=2}^{k}\tau_i \right)b_1
\\
&\geq 
r_1\prod_{i=1}^k\tau_i
+
\frac{B}{1-\otau}
\\
&\geq 
-|r_1|
+
\frac{B}{1-\otau}\triangleq A\leq 0.
\end{align*}
Fix any $\epsilon>0$. Now, since $b_k\to 0$, take some $M$ sufficiently large
so that $b_m\geq -\epsilon(1-\otau)/2$ for all $m\geq M$. Furthermore, pick
some $N$ large enough so that
$
\otau^n A \geq -\epsilon/2
$
for all $n\geq N$.
For all $n\geq N$ and $m\geq M$, we may then write
\begin{align*}
r_{n+m} 
&\geq
\left( \prod_{j=0}^{n-1} \tau_{j+m} \right) r_m 
+ \sum_{j=0}^{n-1}
  \left( \prod_{\ell=j+1}^{n-1} \tau_{\ell+m} \right) b_{j+m} \\
&\geq
\otau^n A 
+ \sum_{j=1}^{n} \otau^{n-j} \big(\! - \epsilon(1-\otau) / 2 \big) \\
&=
\otau^n A 
+ \left( \sum_{j=0}^{n-1} \otau^j \right) \big(\! - \epsilon(1-\otau) / 2 \big) \\
&\geq
\otau^n A 
+ \frac{1}{1-\otau} \big(\! - \epsilon(1-\otau) / 2 \big) 
\geq -\epsilon/2  - \epsilon/2 = -\epsilon.
\end{align*}
Since $\epsilon$ was arbitary, we conclude that $\liminf_{k\to\infty} r_k \geq 0$. 


==> theHyperplane.tex <==


%\section{Weak Convergence of the Asynchronous Algorithm}



% We focus on solving Prob. (\ref{probCompMonoMany}). 

\subsection{Properties of the Hyperplane}\label{secTecLems}\label{secHplane}
Recall that we use $p =(z,\bw) =  (z,w_1,\ldots, w_{n-1})$ for a
generic point in $\bcH$, the collective primal-dual space. For $\bcH$, we
adopt the following norm and inner product for some $\gamma>0$:
\begin{align} \label{gammanorm}
\norm{(z,\bw)}_\gamma^2 &= \gamma\|z\|^2 + \sum_{i=1}^{n-1}\|w_i\|^2 &
\Inner{(z^1,\bw^1)}{(z^2,\bw^2)}_\gamma &= 
   \gamma\langle z^1,z^2\rangle + \sum_{i=1}^{n-1}\langle
w^1_i,w^2_i\rangle.
\end{align}


\begin{lemma}\label{LemGradAffine} Let $\varphi_k$ be defined as in (\ref{hplane}).  Then:
\begin{enumerate}
	\item $\varphi_k$ is affine on $\bcH$. 
	\item \label{item:gradForm} With respect to inner product
	$\langle\cdot,\cdot\rangle_\gamma$ on $\bcH$, the gradient
	of $\varphi_k$ is
	$$
	\nabla\varphi_k =
	\left(\frac{1}{\gamma}\left(\sum_{i=1}^{n-1} G_i^* y_i^k+ y_n^k\right) \!\!,\;
	x_1^k - G_1 x_{n}^k,x_2^k - G_2 x_{n}^k,\ldots,x_{n-1}^k - G_{n-1} x_{n}^k\right).
	$$
	\item 
	Suppose 
	that each $T_i:\calH_i\to2^{\calH_i}$ is monotone and $y_i^k\in T_i x_i^k$ for $i=1,\ldots,n$. Then
	$\varphi_k(p)\leq 0$ for all $p\in \calS$ defined in (\ref{defCompExtSol}).
	\item \label{lem0grad}
   Suppose $y_i^k\in T_i x_i^k$ for $i=1,\ldots,n$, and $\nabla\varphi_k =  0$, then 
    $
    (x_n^k,y_1^k,\ldots,y_{n-1}^k)\in\calS.
    $
\end{enumerate}
\end{lemma}
\begin{proof}
Lemma 4 of \cite{johnstone2018projective}. 
\end{proof}
